CedrusDB: Persistent Key-Value Store with Memory-Mapped Lazy-Trie

As a result of RAM becoming cheaper, there has been a trend in key-value store design towards maintaining a fast in-memory index (such as a hash table) while logging user operations to disk, allowing high performance under failure-free conditions while still being able to recover from failures. This design, however, comes at the cost of long recovery times or expensive checkpoint operations. This paper presents a new in-memory index that is also storage-friendly. A "lazy-trie" is a variant of the hash-trie data structure that achieves near-optimal height, has practical storage overhead, and can be maintained on-disk with standard write-ahead logging. We implemented CedrusDB, persistent key-value store based on a lazy-trie. The lazy-trie is kept on disk while made available in memory using standard memory-mapping. The lazy-trie organization in virtual memory allows CedrusDB to better leverage concurrent processing than other on-disk index schemes (LSMs, B+-trees). CedrusDB achieves comparable or superior performance to recent log-based in-memory key-value stores in mixed workloads while being able to recover quickly from failures.

==> Makefile <==
.PHONE: all clean build

LATEX=pdflatex

FIG_DEPS= \
	figures/hash-trie-overview.tex \
	figures/lazy-trie-compress.tex \
	figures/lazy-trie-split.tex \
	figures/lazy-trie-split-sluggish.tex \
	figures/storage-model-overview.tex \
	figures/node-lock.tex \
	figures/storage-model-space.tex \
	figures/sluggish.pdf \
	figures/zero-copy-value.tex \
	figures/optimistic-logical-space.tex \
	graphs/ycsb-zipfian-k128-nr1e8-no1e8.pdf \
	graphs/ycsb-zipfian-k1024-nr1e7-no1e7.pdf \
	graphs/ycsb-zipfian-k128-nr1e8-no1e8-t4.pdf \
	graphs/ycsb-zipfian-k128-nr1e8-no1e8-aws-concurrent.pdf \
	graphs/ycsb-var-zipfian-k1024-nr1e7-no1e8.pdf \
	graphs/micro-k128-nr1e8-no1e7-t1.pdf \
	graphs/micro-k128-nr1e8-no1e7-t2.pdf \
	graphs/micro-k128-nr1e8-no1e7-t4.pdf \
	graphs/micro-k128-nr1e8-no1e7-hlen-t1.pdf \
	graphs/micro-k128-nr1e8-no1e7-hlen-t4.pdf \
	graphs/micro-elastic-k128-nr1e8-no1e7-t1.pdf \
	graphs/micro-elastic-k128-nr1e8-no1e8-regn-t1.pdf \
	graphs/micro-var-k128-nr1e7-no1e8-t1.pdf \
	graphs/bfactor-sluggishness.pdf

ifeq ($(ARXIV),yes)
	PREFIX=''
	SUFFIX=''
else
	PREFIX='\def\submission{}\input{'
	SUFFIX='}'
endif

all: build

build: paper.tex paper_defs.tex usenix2019_v3.sty $(FIG_DEPS)
	rm -rf _minted-build/ _minted_paper/
	$(LATEX) -jobname=paper -shell-escape $(PREFIX)$<$(SUFFIX)
	bibtex paper
	$(LATEX) -jobname=paper -shell-escape $(PREFIX)$<$(SUFFIX)
	$(LATEX) -jobname=paper -shell-escape $(PREFIX)$<$(SUFFIX)

quick: paper.tex paper_defs.tex usenix2019_v3.sty $(CODE_DEPS) $(FIG_DEPS)
	$(LATEX) -jobname=paper -shell-escape $(PREFIX)$<$(SUFFIX)

paper.pdf: paper.tex paper_defs.tex usenix2019_v3.sty $(CODE_DEPS) $(FIG_DEPS)
	$(LATEX) -jobname=$(basename $@) -shell-escape $(PREFIX)$<$(SUFFIX)

clean:
	rm -rf paper.aux paper.bbl paper.log paper.out paper.pdf paper.blg _minted-build/ _minted-paper/


==> figures/optimistic-logical-space.tex <==
\begingroup
\definecolor{lightorange}{HTML}{ff6929}
\definecolor{lightblue}{HTML}{246aa5}
\definecolor{lightyellow}{HTML}{ffa529}
\definecolor{medgray2}{HTML}{bbbbbb}
\definecolor{medgray}{HTML}{aaaaaa}
\begin{tikzpicture}[x=1.12cm, scale=0.9, every node/.append style={transform shape}]
    \begin{scope}[minimum height=4ex, minimum width=14ex, ]
    \begin{scope}[every node/.append style={drop shadow={shadow xshift=0.3ex,shadow yshift=-0.3ex}, fill=white}]
        \node[draw] (a0) at (0, 0){};
        \node[draw, anchor=west] (a1) at ($(a0.east) + (0.2, 0)$) {};
        \node[draw, anchor=west, dashed] (a2) at ($(a1.east) + (0.2, 0)$) {};
    \end{scope}
    \node[anchor=west] (a3) at ($(a2.east) + (0.2, 0)$) {};
    \begin{pgfonlayer}{lr}
    \clip(-10ex, -3ex) rectangle (6.5, 3ex);
    \node[fit=(a0)(a1)(a2)(a3), draw, line width=0.08ex] (ls) {};
    \end{pgfonlayer}
    \end{scope}
    \node[anchor=south west] at ($(a0.north west) + (0, 0.1)$) {Region $r - 1$};
    \node[anchor=south west] at ($(a1.north west) + (0, 0.1)$) {Region $r$};
    \node[anchor=south west] at ($(a2.north west) + (0, 0.1)$) {Region $r + 1$};
    \begin{scope}[myarrow/.style={decoration={markings,mark=at position 0 with {\arrow[scale=0.8,>=Latex]{<};}}, postaction={decorate}}]
        \draw[myarrow] ($(a1.south) + (0.5, 0.1)$) -- ++(0, -0.5) node (p0) {};
        \draw[myarrow, medgray] ($(a1.south) + (0.6, 0.1)$) -- ++(0, -0.5);
        \draw[myarrow, medgray] ($(a1.south) + (0.7, 0.1)$) -- ++(0, -0.5);
        \draw[myarrow, medgray] ($(a1.south) + (0.8, 0.1)$) -- ++(0, -0.5);
        \draw[myarrow] ($(a1.south) + (0.9, 0.1)$) -- ++(0, -0.5) node (p1) {};
        \draw[myarrow] ($(a1.south) + (1.3, 0.1)$) -- ++(0, -0.5) node (p2) {};
        \draw[myarrow, medgray] ($(a1.south) + (1.4, 0.1)$) -- ++(0, -0.5);
        \draw[myarrow, medgray] ($(a1.south) + (1.5, 0.1)$) -- ++(0, -0.5);
        \draw[myarrow, medgray] ($(a1.south) + (1.6, 0.1)$) -- ++(0, -0.5);
        \draw[myarrow, medgray] ($(a1.south) + (1.7, 0.1)$) -- ++(0, -0.5) node (p3) {};
    \end{scope}
    \begin{scope}[
        draw=lightblue,
        myarrow/.style={%
            decoration={markings,
            mark=at position 0.995 with {\arrow[scale=0.8,>=Latex]{>};}}, postaction={decorate}}]
            \draw[myarrow] (p0.south) to[out=-60,in=-130,looseness=1.7] node[midway, below, xshift=-4ex] {\color{lightblue}{fast path}} (p1.south);
            \draw[myarrow, lightorange] (p1.south) to[out=-60,in=-130,looseness=1.7] node[midway, below, xshift=10ex] {\color{lightorange}{one thread allocates $r + 1$}} (p2.south);
            \draw[myarrow] (p2.south) to[out=-60,in=-130,looseness=1.7] node[midway, below, xshift=-4ex] {} (p3.south);
    \end{scope}
\end{tikzpicture}
\endgroup


==> figures/storage-model-data-space.tex <==
\begingroup
\definecolor{lightorange}{HTML}{ff6929}
\definecolor{lightblue}{HTML}{246aa5}
\definecolor{lightyellow}{HTML}{ffa529}
\definecolor{medgray2}{HTML}{bbbbbb}
\definecolor{medgray}{HTML}{aaaaaa}
\newcommand{\myarray}[6]{%
    \pgfmathsetmacro{\prev}{#1}
    \pgfmathsetmacro{\yy}{0 + #2}
    \pgfmathsetmacro{\yyy}{\yy + #5}
    \tikzstyle{data}=[preaction={transform canvas={shift={(0.4ex,-0.2ex)}},draw=medgray2,very thick}, line width=0.08ex, fill=white]
    \foreach \x/\xs/\c/\b in {#3} {%
        \pgfmathsetmacro{\xx}{\prev}
        \pgfmathsetmacro{\tmp}{\prev + \xs}
        \global\let\prev\tmp
        \draw[draw=black, fill=\c] (\xx * 1ex, \yy * 1ex) rectangle (\prev * 1ex, \yyy * 1ex) node[midway, minimum width=\xs * 1ex, minimum height=#5 * 1ex] (#4a\x) {};
    \ifthenelse{\b = 1}{%
        \draw[draw=black] (\xx * 1ex, \yy * 1ex) -- (\prev * 1ex, \yyy * 1ex) node[midway, minimum width=\xs * 1ex, minimum height=#5 * 1ex] (#4b\x) {};
    }{}

    }
    \pgfmathsetmacro{\pprev}{\prev + #6}
    \draw[draw=black] (\prev * 1ex, \yy * 1ex) -- (\pprev * 1ex, \yy * 1ex) node[midway, minimum height=#5 * 1ex] (#4ax) {};
    \draw[draw=black] (\prev * 1ex, \yyy * 1ex) -- (\pprev * 1ex, \yyy * 1ex) node[midway, minimum height=#5 * 1ex] (#4ax) {};
    \draw[draw=none] (\prev * 1ex, \yy * 1ex) rectangle (\pprev * 1ex, \yyy * 1ex) node[midway, minimum height=#5 * 1ex, minimum width=#6 * 1ex] (#4al) {$\cdots$};
    \begin{pgfonlayer}{bg}
    \draw[] (#1 * 1ex, \yy * 1ex) rectangle (\pprev * 1ex, \yyy * 1ex) node[midway, draw=white, minimum height=#5 * 1ex, minimum width=\pprev * 1ex, drop shadow={shadow xshift=0.3ex,shadow yshift=-0.3ex}, fill=white] (#4ax) {};
    \end{pgfonlayer}
}

\begin{tikzpicture}[x=1.12cm, scale=0.7, every node/.append style={transform shape}]
    \myarray{0}{10}{0/2/white/0,1/2/white/0,2/2/white/0,3/2/white/0,4/2/white/0}{a0}{3}{10}
    \myarray{0}{0}{%
        0/1/lightblue!60/0,
        1/4/white/1,
        2/1/lightyellow!60/0,
        3/1/lightblue!60/0,
        4/10/white/0,
        5/1/lightyellow!60/0,
        6/1/lightblue!60/0,
        7/6/white/1,
        8/1/lightyellow!60/0,
        9/1/lightblue!60/0,
        10/3/white/0,
        11/1/lightyellow!60/0}{a1}{3}{10}
    \begin{scope}[
        myarrow/.style={decoration={markings,mark=at position 1 with {\arrow[scale=0.6,>=Latex]{>};}}, postaction={decorate}}]
        \draw[myarrow] (a0a0.south) -- ++(0, -3ex) -- ++(2ex, 0) -- (a1a1.north);
        \draw[myarrow] (a0a1.south) -- ++(0, -2ex) -- ++(19ex, 0) -- (a1a7.north);
    \end{scope}
    \begin{scope}[densely dashed,
        draw=lightblue,
        myarrow/.style={%
            decoration={markings,
            mark=at position 0.9995 with {\arrow[scale=0.6,>=Latex]{>};}}, postaction={decorate}}]
        \draw[myarrow] (a1a0.north) to[out=90,in=-100] ($(a0a0.south) + (-0.5ex, 0)$);
        \draw[myarrow] (a1a6.north) to[out=90,in=-90,looseness=1.5] ($(a0a1.south) + (-0.5ex, 0)$);
    \end{scope}
    \begin{scope}[densely dashed,
        draw=lightyellow,
        myarrow/.style={%
            decoration={markings,
            mark=at position 0.9996 with {\arrow[scale=0.6,>=Latex]{>};}}, postaction={decorate}}]
        \draw[myarrow] (a1a2.south) to[out=-90,in=-70,looseness=2] (a1a0.south);
        \draw[myarrow] (a1a5.south) to[out=-90,in=-70] (a1a3.south);
        \draw[myarrow] (a1a8.south) to[out=-90,in=-70,looseness=1.5] (a1a6.south);
        \draw[myarrow] (a1a11.south) to[out=-90,in=-70,looseness=2.2] (a1a9.south);
    \end{scope}
    \node[anchor=east] (l1) at (a0a0.west) {descriptors};
    \node[anchor=east] (l2) at (a1a0.west) {data space};
\end{tikzpicture}
\endgroup


==> figures/zero-copy-value.tex <==
\begingroup
\definecolor{lightorange}{HTML}{ff6929}
\definecolor{lightblue}{HTML}{246aa5}
\definecolor{lightyellow}{HTML}{ffa529}
\definecolor{medgray2}{HTML}{bbbbbb}
\definecolor{medgray}{HTML}{aaaaaa}
\newcommand{\myarraya}[6]{%
    \pgfmathsetmacro{\prev}{#1}
    \pgfmathsetmacro{\yy}{0 + #2}
    \pgfmathsetmacro{\yyy}{\yy + #5}
    \tikzstyle{data}=[preaction={transform canvas={shift={(0.4ex,-0.2ex)}},draw=medgray2,very thick}, line width=0.08ex, fill=white]
    \pgfmathsetmacro{\pprev}{\prev + #6}
    \draw[draw=black] (\prev * 1ex, \yy * 1ex) -- (\pprev * 1ex, \yy * 1ex) node[midway, minimum height=#5 * 1ex] (#4ay) {};
    \draw[draw=black] (\prev * 1ex, \yyy * 1ex) -- (\pprev * 1ex, \yyy * 1ex) node[midway, minimum height=#5 * 1ex] (#4ay) {};
    \draw[draw=none] (\prev * 1ex, \yy * 1ex) rectangle (\pprev * 1ex, \yyy * 1ex) node[midway, minimum height=#5 * 1ex, minimum width=#6 * 1ex] (#4ar) {$\cdots$};
    \pgfmathsetmacro{\prev}{\pprev}
    \foreach \x/\xs/\b in {#3} {%
        \pgfmathsetmacro{\xx}{\prev}
        \pgfmathsetmacro{\tmp}{\prev + \xs}
        \global\let\prev\tmp
        \ifthenelse{\b = 1}{%
            \draw[draw=black, fill=lightblue!50] (\xx * 1ex, \yy * 1ex) rectangle (\prev * 1ex, \yyy * 1ex) node[midway, minimum width=\xs * 1ex, minimum height=#5 * 1ex] (#4a\x) {};
        }{
            \draw[draw=black] (\xx * 1ex, \yy * 1ex) rectangle (\prev * 1ex, \yyy * 1ex) node[midway, minimum width=\xs * 1ex, minimum height=#5 * 1ex] (#4a\x) {};
        }
    }
    \pgfmathsetmacro{\pprev}{\prev + #6}
    \draw[draw=black] (\prev * 1ex, \yy * 1ex) -- (\pprev * 1ex, \yy * 1ex) node[midway, minimum height=#5 * 1ex] (#4ax) {};
    \draw[draw=black] (\prev * 1ex, \yyy * 1ex) -- (\pprev * 1ex, \yyy * 1ex) node[midway, minimum height=#5 * 1ex] (#4ax) {};
    \draw[draw=none] (\prev * 1ex, \yy * 1ex) rectangle (\pprev * 1ex, \yyy * 1ex) node[midway, minimum height=#5 * 1ex, minimum width=#6 * 1ex] (#4al) {$\cdots$};
    \begin{pgfonlayer}{bg}
    \draw[] (#1 * 1ex, \yy * 1ex) rectangle (\pprev * 1ex, \yyy * 1ex) node[midway, draw=white, minimum height=#5 * 1ex, minimum width=\pprev * 1ex, drop shadow={shadow xshift=0.3ex,shadow yshift=-0.3ex}, fill=white] (#4ax) {};
    \end{pgfonlayer}
}

\newcommand{\myarrayb}[5]{%
    \pgfmathsetmacro{\prev}{#1}
    \pgfmathsetmacro{\yy}{0 + #2}
    \pgfmathsetmacro{\yyy}{\yy + #5}
    \tikzstyle{data}=[preaction={transform canvas={shift={(0.4ex,-0.2ex)}},draw=medgray2,very thick}, line width=0.08ex, fill=white]
    \foreach \x/\xs/\b in {#3} {%
        \pgfmathsetmacro{\xx}{\prev}
        \pgfmathsetmacro{\tmp}{\prev + \xs}
        \global\let\prev\tmp
        \draw[draw=black, fill=lightblue!50] (\xx * 1ex, \yy * 1ex) rectangle (\prev * 1ex, \yyy * 1ex) node[midway, minimum width=\xs * 1ex, minimum height=#5 * 1ex] (#4a\x) {};
        \ifthenelse{\b = 1}{%
            \draw[draw=black] (\xx * 1ex, \yy * 1ex) -- (\prev * 1ex, \yyy * 1ex) node[midway, minimum width=\xs * 1ex, minimum height=#5 * 1ex] (#4b\x) {};
        }{}
    }
    \begin{pgfonlayer}{bg}
    \draw[] (#1 * 1ex, \yy * 1ex) rectangle (\prev * 1ex, \yyy * 1ex) node[midway, draw=white, minimum height=#5 * 1ex, minimum width=(\prev - #1) * 1ex, drop shadow={shadow xshift=0.3ex,shadow yshift=-0.3ex}, fill=white] (#4ax) {};
    \end{pgfonlayer}
}

\begin{tikzpicture}[x=1.12cm, scale=0.9, every node/.append style={transform shape}]
    \myarraya{0}{10}{0/6/1,1/6/0,2/6/1,3/6/1,4/6/0,5/6/1,6/6/0,7/6/1}{a0}{3}{6}
    \myarrayb{15}{0}{0/6/0,1/6/0,2/6/0,3/6/0,4/6/0}{a1}{3}
    \begin{scope}[myarrow/.style={decoration={markings,mark=at position 1 with {\arrow[scale=1]{>};}}, postaction={decorate}}]
        \draw[myarrow, lightblue] ([xshift=-1ex] a0a0.south) -- ++(0, -0.65) -| ([xshift=-1ex] a1a0.north);
        \draw[myarrow, lightblue] ([xshift=-1ex] a0a2.south) -- ++(0, -0.65) -| ([xshift=-1ex] a1a1.north);
        \draw[myarrow, lightblue] ([xshift=-1ex] a0a3.south) -- ++(0, -0.65) -| ([xshift=-1ex] a1a2.north);
        \draw[myarrow, lightblue] ([xshift=-1ex] a0a5.south) -- ++(0, -0.45) -| ([xshift=-1ex] a1a3.north);
        \draw[myarrow, lightblue] ([xshift=-1ex] a0a7.south) -- ++(0, -0.45) -| ([xshift=-1ex] a1a4.north);

        \draw[myarrow, orange] ([xshift=1ex] a1a0.north) -- ++(0, 0.65) -| ([xshift=1ex] a0a0.south);
        \draw[myarrow, orange] ([xshift=1ex] a1a1.north) -- ++(0, 0.65) -| ([xshift=1ex] a0a2.south);
        \draw[myarrow, orange] ([xshift=1ex] a1a2.north) -- ++(0, 0.65) -| ([xshift=1ex] a0a3.south);
        \draw[myarrow, orange] ([xshift=1ex] a1a3.north) -- ++(0, 0.45) -| ([xshift=1ex] a0a5.south);
        \draw[myarrow, orange] ([xshift=1ex] a1a4.north) -- ++(0, 0.45) -| ([xshift=1ex] a0a7.south);
    \end{scope}
    \node[anchor=south west] (l1) at (a0a0.north west) {block data space};
    \node[anchor=north west] (l2) at (a1a0.south west) {temporary value space};
\end{tikzpicture}
\endgroup

